LOTUS: Continual Imitation Learning for Robot Manipulation Through Unsupervised Skill Discovery

We introduce LOTUS, a continual imitation learning algorithm that empowers a physical robot to continuously and efficiently learn to solve new manipulation tasks throughout its lifespan. The core idea behind LOTUS is constructing an ever-growing skill library from a sequence of new tasks with a small number of human demonstrations. LOTUS starts with a continual skill discovery process using an open-vocabulary vision model, which extracts skills as recurring patterns presented in unsegmented demonstrations. Continual skill discovery updates existing skills to avoid catastrophic forgetting of previous tasks and adds new skills to solve novel tasks. LOTUS trains a meta-controller that flexibly composes various skills to tackle vision-based manipulation tasks in the lifelong learning process. Our comprehensive experiments show that LOTUS outperforms state-of-the-art baselines by over 11% in success rate, showing its superior knowledge transfer ability compared to prior methods. More results and videos can be found on the project website: https://ut-austin-rpl.github.io/Lotus/.

==> tmp_background.tex <==
% \yifeng{Not sure if we want to have a background session.}

% \yifeng{Shorten this and do a lifelong learning formulation.}

% \begin{enumerate}
%     \item \yifeng{This section should introduce base task / lifelong learning task stage}
%     \item \yifeng{In this section, we also mention that at lifelong learning task stage, we can have a group of new tasks at each stage. But in our method description, we assume one new task at each stage to simplify the notation and description.}
% \end{enumerate}
We introduce the backgrounds of vision-based robot manipulation and lifelong imitation learning in order to formulate the continual skill discovery problem in robot manipulation.

\myparagraph{Vision-Based Manipulation as Markov Decision Process}
We formulate a vision-based robot manipulation task as a finite-horizon Markov Decision Process:
$
\mathcal{M} = (\mathcal{S}, \mathcal{A}, \mathcal{T}, H, \mu_0, R)
$. Here,
$\mathcal{S}$ is the space of the robot's raw sensory data, including RGB images and proprioception. $\mathcal{A}$ is the space of the robot’s motor commands. $\mathcal{T}: \mathcal{S}\times \mathcal{A} \mapsto \mathcal{S}$ is transition dynamics.  $H$ is the maximal horizon for each episode of tasks. $\mu_0$ is the initial state distribution. $R(s,a,s')$ is the reward function. We consider a sparse-reward setting, where the reward function is defined by a goal predicate $g:\mathcal{S}\mapsto \{0, 1\}$. The robot's ultimate objective is to learn a policy $\pi$ that maximizes the expected return:
$
\max_\pi J(\pi) = \mathbb{E}_{s_t, a_t \sim \pi, \mu_0} [\sum_{t=1}^{H} g(s_t)].
$

% \subsection{Lifelong Imitation Learning For Robot Manipulation}
\myparagraph{Lifelong Robot Learning Problem.} In a \emph{lifelong robot learning problem}, a robot sequentially learns a policy $\pi$ over $\maxtasknum$ tasks $\{T^{\tasknum}\}_{\tasknum=1}^{\maxtasknum}$. We assume $\pi$ is conditioned on the task, i.e., $\pi(\cdot|s; T)$. Each task $T^\tasknum \equiv (\mu_0^\tasknum, g^\tasknum)$ is defined by the initial state distribution $\mu_0^\tasknum$ and the goal predicate $g^\tasknum$. During lifelong learning, a robot might experience a number of tasks indexed from $\tasknum_{c-1}$ to $\tasknum_{c}$ at a time $c$ in a lifelong learning sequence with a total length of $C$. Concretely, a robot will learn over a lifelong learning sequence $T^{1:\tasknum_{1}}$, $T^{\tasknum_{1}:\tasknum_{2}}$, \dots, $T^{\tasknum_{C-1}:\tasknum_{C}}$, where $1<\tasknum_{c}<\maxtasknum (1\leq c < C)$ and $\tasknum_{C}=\maxtasknum$. We can break the lifelong learning sequence into two parts, a \textit{base task stage} for learning a multitask policy over $T^{\tasknum_{0}:\tasknum_{1}}$, and a \textit{lifelong task stage} where a robot sequentially learns all the other tasks $T^{\tasknum_{1}:\maxtasknum}$. For clarity of presentation, the rest of the descriptions in Section~\ref{sec:background} and~\ref{sec:method} assume one task is learned at a time during the lifelong task stage. 

We assume $\mathcal{S}, \mathcal{A}, \mathcal{T}, H$ are the same for all tasks. Up to the $\tasknum$-th task $T^\tasknum$, the robot aims to optimize
\begin{equation*}
    \max_\pi~ J_{\text{LRL}}(\pi) = \frac{1}{\tasknum}\sum_{p=1}^\tasknum \bigg[ \mathop{\mathbb{E}}\limits_{s^p_t, a^p_t \sim \pi(\cdot;T^p),~ \mu_0^p} \bigg[\sum_{t=1}^L g^p(s_t^p) \bigg] \bigg]
    \label{eq:LRL}
\end{equation*}
During the lifelong learning process, the robot agent loses access to any data from the previous $\tasknum-1$ tasks when it is trained on task $T^{\tasknum}$.

\myparagraph{Lifelong Imitation Learning.} As we mention in Sec.~\ref{sec:intro}, we consider a lifelong imitation learning setting that allows sample efficient policy learning over tasks with sparse rewards. For each task $T^{\tasknum}$, a robot is provided with a small dataset of $\maxdemo$ demonstrations for $T^{\tasknum}$, denoted as $D^{\tasknum}=\{\tau^{\tasknum}_{i}\}_{i=1}^{\maxdemo}$. $T^{\tasknum}$ also comes with a language description $l^{\tasknum}$ that uniquely identifies a task. 
In this paper, we assume demonstrations are collected through expert teleoperation. Each demonstration trajectory consists of state action pairs  $\tau^{\tasknum}_{i}=\{(s_{t}, a_{t})\}_{t=1}^{t_{\tasknum}}$ where $t_{\tasknum} < H$. We train the policy $\pi$ using behavioral cloning~\cite{bain1995framework} with a surrogate objective: 
\begin{equation*}
 \min_\pi~ J_{\text{BC}}(\pi) = \frac{1}{\tasknum}\sum_{p=1}^\tasknum \mathop{\mathbb{E}}\limits_{o_t, a_t \sim D^p} \bigg[ \sum_{t=0}^{l^p} \mathcal{L}_{\text{BC}}\big(\pi(o_{\leq t}; l^p), a^p_t\big)\bigg]\,
    \label{eq:bc}
\end{equation*}
where $\mathcal{L}_{\text{BC}}$ is a supervised behavior cloning loss. During the lifelong learning process, the robot agent loses full access to $\{D^p: p < \tasknum\}$ when learning $T^\tasknum$, rendering naive multitask learning methods not applicable in lifelong learning.

To evaluate the performance of policy $\pi$ over the lifelong learning process, we use three standard metrics used in prior works~\cite{lopez2017gradient,diaz2018don,liu2023libero}: FWT (forward Transfer), NBT (negative backward transfer), and AUC (area under the success rate curve). All three metrics are computed in terms of success rates, where a higher FWT suggests quicker adaptation to new tasks, a lower NBT indicates better performance on past tasks, and a higher AUC reflects overall performance considering both metrics. Intuitively, the AUC metric can be interpreted as a surrogate metric to quantify the average success rates during the entire lifelong learning process. Denote $r_{i, j}$ as the agent's success rates on task $j$ when it has just learned over previous $i$ tasks. Following the metric definition in LIBERO, we have: $\text{FWT}=\sum_{\tasknum\in[\maxtasknum]}\frac{r_{\tasknum, \tasknum}}{\maxtasknum}$, $\text{NBT}=\sum_{\tasknum\in[\maxtasknum]}\frac{\text{NBT}_{\tasknum}}{\maxtasknum}$, $\text{NBT}_{\tasknum}=\frac{1}{\maxtasknum - \tasknum}\sum_{q=\tasknum+1}^{\maxtasknum}(r_{\tasknum, \tasknum}, r_{q, \tasknum})$, and $\text{AUC}=\sum_{\tasknum\in[\maxtasknum]}\frac{\text{AUC}_{\tasknum}}{\maxtasknum}$, $\text{AUC}_{\tasknum}=\frac{1}{\maxtasknum - \tasknum + 1}(r_{\tasknum, \tasknum} + \sum_{q=\tasknum+1}^{\maxtasknum}r_{q, \tasknum})$.



% \subsection{Evaluation Metrics}
% To evaluate the lifelong learning task stage, following~\cite{diaz2018don, liu2023libero}, we use FWT (forward Transfer), NBT (negative backward transfer), and AUC (area under the success rate curve) as the evaluation metrics which are all computed in terms of success rate. 
% A lower NBT indicates better performance on past tasks, while a higher FWT suggests quicker adaptation to new tasks. A higher AUC reflects overall superior performance considering both metrics.
% Denote $c_{i,j,e}$ as the agent’s success rate on task $j$ when it learned over $i−1 $previous tasks and has just learned $e$ epochs on task $i$. 
% On current task $i$, $c_{i,i} = \max_{e}c_{i,i,e}$ is the best success rate over all
% evaluated epochs, and $e^{*}_i = \arg\min_{e} c_{i,i,e_i} = c_{i,i}$ is the earliest epoch to achieve the best performance.
% For task $j\neq i$, we define $c_{i,j} = c_{i,j,e^∗_i}$.
% Same as LIBERO~\cite{liu2023libero}, we assume all $e \geq e^*_i, c_{i,i,e} = c_{i,i}$. 
% Following this annotation, we have:
% $\text{FWT} = \sum_{\tasknum\in[\maxtasknum]} \frac{\text{FWT}_\tasknum}{\maxtasknum},~~~\text{FWT}_\tasknum = \frac{1}{11}\sum_{e \in \{0 \dots 50\}} c_{\tasknum,\tasknum,e}$, 
% $\text{NBT} = \sum_{\tasknum\in[\maxtasknum]} \frac{\text{NBT}_\tasknum}{\maxtasknum},~~~~\text{NBT}_\tasknum =  \frac{1}{\maxtasknum-\tasknum} \sum_{\tau = \tasknum+1}^\maxtasknum \big(c_{\tasknum, \tasknum} - c_{\tau, \tasknum}\big)$, and
% $\text{AUC} = \sum_{\tasknum\in[\maxtasknum]} \frac{\text{AUC}_\tasknum}{\maxtasknum},~~~\text{AUC}_\tasknum =\frac{1}{\maxtasknum-\tasknum+1} \big(\text{FWT}_\tasknum + \sum_{\tau=\tasknum+1}^\maxtasknum c_{\tau, \tasknum}\big)$.


% where a small demonstration dataset is provided for every task in the lifelong learning sequence. Demonstrations allow sample efficient policy learning in sparse-reward settings, which is a great challenge for reinforcement learning approaches. 

% several base tasks $\{T^1, \dots, T^{\maxtasknum_0}\}$ at the beginning, and then in the lifelong stage, we would be provided with a small demonstration dataset for each new task sequentially, following the order in the sequence $\{T^{\maxtasknum_0+1}, \dots, T^{\maxtasknum}\} (\maxtasknum_0 < \maxtasknum)$.


% We denote $\{T^1, \dots, T^{\maxtasknum_0}\}$ as the base task set and $\{T^{\maxtasknum_0+1}, \dots, T^{\maxtasknum}\}$ as the lifelong learning task set. 

% \myparagraph{Lifelong Imitation Learning} As we mention in Section~\ref{sec:intro}, we follow the convention of LIBERO~\cite{liu2023libero}, where a small demonstration dataset is provided for every task in the lifelong learning sequence. Demonstrations allow sample efficient policy learning in the sparse-reward settings, which is a great challenge for reinforcement learning approaches. 

% In this work, due to the challenge of sparse-reward setting, we consider a \emph{lifelong imitation learning problem} setting that is sample efficient: we assume we are provided with some demonstrations of several base tasks $\{T^1, \dots, T^{\maxtasknum_0}\}$ at the beginning, and then in the lifelong stage, we would be provided with a small demonstration dataset for each new task sequentially, following the order in the sequence $\{T^{\maxtasknum_0+1}, \dots, T^{\maxtasknum}\} (\maxtasknum_0 < \maxtasknum)$. We aim to solve this new task while preserving knowledge of previous tasks. Thus, this process unfolds in two stages: 1) base task stage; 2) lifelong learning task stage.
% In practice, during the lifelong learning task stage, multiple new tasks can emerge at each stage. However, for clarity in notation and description within our method, we assume the introduction of a single new task at each stage.
% Denote $D^\tasknum = \{ \tau^\tasknum_i \}_{i=1}^\maxdemo$ as $\maxdemo$ demonstrations for task $T^\tasknum$.  Each $\tau^\tasknum_i = (o_0, a_0, o_1, a_1, \dots, o_{l^\tasknum})$ where $l^\tasknum \leq H$. Here, $o_t$ is the robot's sensory input, including the perceptual observation and robot proprioception. 
% % In practice, the observation $o_t$ is often non-Markovian. Therefore
% We represent $s_t$ by the aggregated history of observations, i.e. $s_t \equiv o_{\leq t} \triangleq (o_0, o_1, \dots, o_t) $.
% % This results in the \emph{lifelong imitation learning problem} with the same objective as in Eq.~\eqref{eq:LRL}. But 
% During training, we perform behavioral cloning~\citep{bain1995framework} with the following surrogate objective function:
% \begin{equation}
%  \min_\pi~ J_{\text{BC}}(\pi) = \frac{1}{\tasknum}\sum_{p=1}^\tasknum \mathop{\mathbb{E}}\limits_{o_t, a_t \sim D^p} \bigg[ \sum_{t=0}^{l^p} \mathcal{L}_{\text{BC}}\big(\pi(o_{\leq t}; T^p), a^p_t\big)\bigg]\,,
%     \label{eq:bc}
% \end{equation}
% where $\mathcal{L}$ is the supervised behavior cloning loss. We assume $\{D^p: p < \tasknum\}$ are not fully available when learning $T^\tasknum$.



==> tmp_method.tex <==

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth, trim=0cm 0cm 0cm 0cm,clip]{figures/Method.pdf}
    \vspace{-1mm}
    \caption{Overview of \ourmethod{}. }
    \label{fig:method-overview}
    \vspace{-4mm}
%\end{minipage}
\end{figure*}

\weikang{$\{\tilde{D^i}, i=0,1,2...,k_n\}$ indicate skill dataset at lifelong stage $n$, maximum lifelong stage N}

We present \ourmethod{}, a novel algorithm for lifelong skill discovery in vision-based robot manipulation. The core idea of this approach is constructing an ever-increasing library of robot skill policies. Throughout the lifelong learning process, the skill library continually adds new skills while existing skills are refined. The overview of \ourmethod{} is shown in Figure~\ref{fig:method-overview}. We first provide the general formulation of lifelong skill discovery. Then we introduce two major components that \ourmethod{} implements: continual skill clustering with an open-vocabulary model and hierarchical policy learning where we train an ever-increasing skill library and a meta controller that invokes the skills. 
% For a new task, several skills are reused, as well as learning new skills, which significantly accelerates learning the new task while preserving knowledge of previous tasks. 


\subsection{Formulation of Lifelong Skill Discovery}
\yifeng{Formulate skill discovery problem based on the lifelong imitation learning formulation we had in the background section.
\begin{enumerate}
    \item How we partition demonstrations into skill datasets in the lifelong learning context.
    \item We need to emphasize that the datasets from previous tasks won't be available. We employ an approach based on experience replay, which allows to save a very small amount of data that are significantly smaller than the number of demonstrations given.
    \item Represent robot policies as hierarchical policies.
\end{enumerate}
}

\change{To leverage the inductive of skills that are shared across different tasks,} we consider a hierarchical policy learning paradigm, where we factorize the policy $\pi$ with a two-level hierarchy: the low level consists of a set of skills from the ever-increasing skill library $\skillpolicy{}$ and the high level is a meta controller $\metacontroller{}$ that invokes the skills. At lifelong learning step $c$, the factorized policy can be written as: $\pi(a_t|s_t,l) = \metacontroller{}(\param_t,k_t|s_t,l)\skillpolicy{k_{t}}(a_t|s_t,\param_t)$, where $l\in \{l^{\tasknum}\}_{\tasknum=1}^{\maxtasknum_{C}}$, $k_t \in [K_{c}]$, $\omega_{t}$ is the subgoal parameter. The goal of the life skill discovery problem is to find the skill library $\skillpolicy{}$  that continually increases over a sequence of demonstrations. At a lifelong learning step $c$, demonstrations of new tasks are divided into maximally $K_{c}$ partitions, where $K_{c}$ is the maximal number of skills until step $c$. Each partition is used to fine-tune an existing policy or train a new policy if the partition does not exist before step $c$. If a partition does not have any new data, its corresponding policy remains fixed. At the base task stage, the lifelong skill discovery problem is equivalent to multitask skill discovery, where we initialize the skill library and the meta controller for the subsequent lifelong learning steps.

In the lifelong learning setting, demonstration datasets from previous tasks won't be fully available. In this work, we use experience replay for policy learning that has a memory buffer to save a portion of data significantly smaller than the size of demonstration datasets.


% ---------------我是华丽的分割线------------------

We present the formulation of lifelong skill discovery from demonstrations. Given a sequence of tasks during lifelong learning, lifelong skill discovery continually identifies skills from the demonstration accompanying the tasks. At every step $n$ of lifelong learning, new demonstrations are divided into $K_n$ partitions, where each partition will be identified if a new skill should be created. 

We first identify the set of multitask demonstrations 

Note that at the base task stage, the lifelong learning just starts and the robot has full access to the complete set of demonstrations. In this case, the skill discovery essential functions as multitask skill discovery. 

In the base task stage, we assume 50 tasks for each task. We divide the task dataset $\{D^\tasknum, m=0,1,...,T^{\maxtasknum_0}\}$ into skill dataset $\{\tilde{D^i}, i=0,1...,k_0\}$ using our skill discovery method. 
Within the lifelong learning task stage, we assume 10 tasks for each new task and we store 5 demonstrations in the skill dataset for each old task. Throughout the lifelong learning task stage, the skill dataset is continually updated as new task demonstrations are added. Following skill discovery at the stage $n$, the skill dataset becomes $\{\tilde{D^i}, i=0,1...,k_n\}$.
Following BUDS~\cite{zhu2022bottom}, we use a two-level hierarchical policy architecture. First, we train each skill $\skillpolicy{i}, i\in\{1,2,...,k_n\}$ on its corresponding dataset $\tilde{D^i}$. The input of the skill policy $\skillpolicy{i}(a_t|s_t,z_t,\languagegoal{})$ are sensor observation $s_t$, subgoal embedding $z_t$, and language instruction $l$. We then train a high-level meta-controller policy $\metacontroller{i}(z_t,h_t|s_t,l)$ to predict the skill index $h_t=i$ and skill parameter (or called subgoal embedding) $z_t$. The whole policy can be factorized as $\pi(a_t|s_t,l) = \metacontroller{}(z_t,h_t, i|s_t,l)\skillpolicy{i}(a_t|s_t,z_t,l)$.


\subsection{Open-vocabulary Models For Temporal Segmentation}
\label{sec:04-discovery}
% 1. First give an overview of the skill discovery process
Given a new task $T^k$ and several demonstrations $D^k$ of this task, our objective is to identify the hierarchical structures of these demonstrations and discover temporal segments in the demonstrations.
Leveraging the bottom-up skill discovery approach from BUDS~\cite{zhu2022bottom}, we effectively group per-frame representations based on temporal proximity to establish a tree structure of segments, which serves as a hierarchical representation of demonstration sequences. Specifically, we use the hierarchical agglomerative clustering method. Beginning with the foundational segments of length $W$, at each iteration, we select two adjacent segments based on the cosine similarity of their features among all pairs of adjacent segments and then merge them into an elongated segment. This process is reiterated until all segments coalesce into a singular segment for each demonstration. Once we obtain the tree structure for every demonstration, we identify intermediate segments referred to as temporal segments following BUDS.\weikang{do we need to explain temporal segments and this process?}
% we identify intermediate segments referred to as temporal segments—by performing a breadth-first search starting from the root node of the hierarchy. This entire breadth-first search is halted once the count of temporal segments surpasses a predetermined threshold.

% 2. Insights on introducing open-vocabulary models

% 3. What is required for temporal segmentation in lifelong learning process --- consistent criteria for segmenting temporally-extended trajectory -> a model that captures consistent semantic meaning, and thus a model that can naturally indiciate "event changes" without assuming a fixed set of distributions.

One critical question is how to obtain the representation of each frame. Throughout the lifelong learning process, we continually encounter new tasks. The image feature distribution between these new tasks and previous ones might vary considerably. Much of the prior works~\cite{nasiriany2022learning,pertsch2021accelerating,zhu2022bottom} has operated under the assumption that, in a multi-task setting. BUDS trained a multi-sensory state representations encoder over the complete multi-task dataset by a reconstruction task, aiming to extract the representation of each state. However, in a lifelong learning scenario, we cannot anticipate the data from future tasks. Furthermore, training a separate encoder for each new task to extract features would not only increase the cost throughout the lifelong learning process, but the demonstration segment for each task would also be inconsistent, which is not conducive to subsequent skill clustering and learning. 
Therefore, what is imperative for temporal segmentation in the lifelong learning process is a consistent criterion for segmenting temporally-extended trajectories. A model is required that captures a consistent semantic meaning, enabling it to naturally indicate "event changes" without assuming a fixed distribution set. Open-vocabulary models such as DINOv2~\cite{oquab2023dinov2}, CLIP~\cite{radford2021learning}, and OWL-ViT~\cite{minderer2022simple}, trained on vast datasets, demonstrate robust generalization capabilities. These models have showcased potent zero-shot capabilities in downstream visual tasks, including classification, instance recognition, and video classification. Consequently, we employ the DINOv2 model to extract per-frame representations. Specifically, we concatenate the global DINOv2 features of images obtained from two camera views within the same frame, using these as the current frame's features. Utilizing the DINOv2 feature space ensures that all temporal segmentations during the lifelong process have a consistent segmentation basis and a strong, consistent semantic meaning.

\subsection{Continual Learning of Skill Library}
\label{sec:04-skills}

% 1. Overview: This part will decide if a new skill is needed, or new data will be incorporated into old skills.

% 2. Proposed algorithm to decide if new data should be included in existing skills or add a new skills

% 3. Mention how we compute the feature of every temporal segment to do the skill clustering

% 4. Then describe that how we prepare the datasets for each skills. 

% 5. Mention that we do experience replay, so we do not store all the raw data. In the clustering step, we only store the computed features of temporal segments, which has neglegible memory cost compared to comparing all data in temporal segments.

We build a skill library, wherein demonstrations from diverse tasks are clustered and partitioned. Subsequently, an individual skill policy is trained on each clustered dataset. Throughout the lifelong learning process, there's a consistent update to the data and skill policy contained within the entire skill library.

To begin, for all temporal segments, we compute the DINOv2 feature for every image frame within a segment. This is followed by the employment of global pooling to ascertain the feature representation of this segment. This global pooling feature stands as the signature attribute of a temporal segment. Robot skill semantics are inherently encapsulated within segments; hence, discerning similarities and disparities among segments necessitates features that elucidate their semantic differences across temporal frames. The global pooling operation provides a computationally efficient way to aggregate information on robot actions across all frames and capture the semantics of manipulation behaviors. This diverges from the design adopted in previous studies where solely heuristically chosen image frames were utilized to compute a segment's feature, resulting in the loss of temporal continuity and the dynamic essence intrinsically embedded in the segment.

During the Multi-task Learning stage, we leverage the global feature of temporal segments as the clustering criterion. Using spectral clustering, we partition all temporal segments into $k_0$ groups. We use the Silhouette method~\cite{rousseeuw1987silhouettes} to determine the optimal number of clusters $k_0$ which then defines the number of skills in the initial skill library. Each cluster $i$, comprising all segments' data, is perceived as a skill dataset $\tilde{D^i}$ for a distinct skill $i$. On this foundation, we train a Transformer-based skill policy for each skill.

In the lifelong task stage, we do not store all the raw data. During the clustering procedure, only the computed features of the temporal segments are retained. This approach incurs a negligible memory cost compared to storing all data within temporal segments. For demonstrations of a new task, we use the same hierarchical clustering method with DINOv2 model to derive a series of temporal segments and their corresponding global features. For each temporal segment, its global feature is compared against the Silhouette value of every existing cluster. \yifeng{We need to cite Silhouette method and explain first what is the high level intuition of Silhouette value (What does it quantify, and why is ti a good option for quantify in our skill clustering result.)} \yifeng{Also emphasize that in practice, we found that the threshold can be easily determined and the clustering result is resilient to a wide range of values.} If this value falls below a set threshold, a new skill cluster is instantiated for the current segment. Otherwise, the data is allocated to the cluster exhibiting the maximum Silhouette value.\weikang{Do we need to write the mathematical form of this?} At the lifelong stage $n$, once this procedure is executed for all segments of the new task demonstrations, new skill cluster data may be introduced and old skill data will be updated. Finally, we get an updated skill dataset $\{\tilde{D^i}, i=0,1,2...,k_n\}$, where $k_n$ is the max skill index at the lifelong stage $n$. 
Following the updates to the skill dataset in the skill library, skill policies linked to altered cluster data undergo \cofinetuning using the Experience Replay (ER)~\cite{chaudhry2019tiny} method, while newly introduced skills are trained from scratch. 
ER samples data from memory, amalgamating it with the current task's training data to ensure the training dataset closely mirrors the empirical distribution across all tasks. 
In our implementation, we use 5 demonstrations for each old task and 10 demonstrations for the new task to \cofinetune the skill policies. After training, 5 out of the 10 demonstrations for the new task are restored.

\subsection{Hierarchical Policies in Lifelong Learning}
\label{sec:04-hierarchical}

% 1. Explain how meta-controllers accommodate increasing number of skills

% 2. Briefly explain cVAE for predicting skill id, and subgoal parameters.

% 3. Also mention that the meta controller is now a transformer-based architecture, which is different from the original design in BUDS.

% 4. mention that now it's only a single meta controller. Explain why not BUDS original design --- The number of meta controllers will be unbounded in lifelong scenario if we learn a single meta controller each time, thus used a single model but conditioned on language instruction instead.

% 5. Then explain how we perform experience replay on both meta-controller and skill policies.

% Tentative item: if we can get results of ablation on ER with tabula rasa meta controllers, then we can make stronger claim about fine-tuning meta controllers with ER method (it also leverages the prior knowledge about skill composition).






\weikang{need to be consistent with method figure, e.g., policy inpput}
\yifeng{We also need to mention about memory buffer.}
In the skill policy $\skillpolicy{i}$, we learn a latent space $\Omega$ for subgoal embeddings. We define the subgoal of time step $t$ as the sensor observation either $T$ steps ahead of $s_t$ in the demonstration or the last state of a temporal segment if it reaches the end of the segment from $s_t$  within $T$ steps. We generate a latent subgoal embedding $z_t$ for the subgoal $s_{g_t}$ at time step $t$, using a subgoal encoder.
We define a subgoal as a look-ahead visual observation fixed at a constant number of steps ahead, rather than the final goal state of the task. This approach is motivated by the desire to leverage temporal abstraction, thereby mitigating the computational overhead associated with individual skill execution. Consequently, skills are oriented towards achieving short-horizon subgoals, obviating the necessity for intricate reasoning about long-term objectives.
As Fig~\ref{fig:method-overview} shows, the skill policy architecture integrates visual, temporal, and linguistic information. We use ResNet as the visual backbone that encodes current visual observations and subgoal visual observations to visual tokens. Language instructions of tasks are encoded to a language token using pretrained BERT embeddings~\cite{devlin2018bert}. The language instruction is also incorporated into the ResNet features using the FiLM method~\cite{perez2018film}. We use a Transformer encoder~\cite{liu2023libero,zhu2022viola,vaswani2017attention} as the temporal backbone to process a temporal sequence of tokens.
Note that the language embedding and subgoal embedding are treated as separate tokens in inputs to the transformer alongside. 
For each decision-making step, our temporal backbones output a latent vector representation. To compute the multi-modal distribution over manipulation actions, we use a Gaussian Mixture Model(GMM) based output head~\cite{mandlekar2021matters,bishop1994mixture}. We use the negative log-likelihood behavior cloning loss to train the skill policies.

For the high-level meta-controller policy $\metacontroller{}(z_t,h_t|s_t,l)$, we use a similar network backbone to the skill policy. Instead of directly predicting the skill index $h_t$ and the subgoal embedding $z_t$ on top of the transformer output latent vector, we use a conditional Variational Autoencoder (cVAE)~\cite{kingma2013auto}. This is motivated by the fact that human demonstrations are multi-modal and contain multiple modes of behavior~\cite{grauman2022ego4d,lynch2020learning}.
The meta-controller is trained to generate a skill index $h_t$ and the subgoal embedding $z_t$ using ELBO loss following the cVAE training convention in previous works~\cite{mandlekar2020learning,zhu2022bottom}.
\yifeng{Insights on why only using workspace images and proprioception in meta controllers --- related to our insights on how to identify skill semantics and its goals: the decision of invoking which skills and the subgoals majorly depends on the holistic semantics of the scene and the robots' own joint motion. Eye-in-hand cameras are majorly useful for precise control, as also shown in prior work~\cite{}.  }
For the input sensor observation $s_t$ of the $\metacontroller{}$, we only use the workspace (AgentView) image and proprioception. This choice stems from our insights into skill semantics and goal identification: the selection of appropriate skills and subgoals chiefly relies on the overarching scene semantics and the robot's own joint movements. As shown in prior research~\cite{}, eye-in-hand cameras are predominantly advantageous for precision control.


Throughout the lifelong learning process, our approach continuously incorporates new skills into the skill library while simultaneously refining existing ones. This augmentation and refinement are achieved by training new skill policies from scratch and \cofinetuning \weikang{can we use this word?} previously established skills using Experience Replay. For the high-level meta-controller, considering that the range of the skill index can vary throughout the lifelong process, we assume a maximum potential skill count of $Q >>k_N$. Thus, the meta-controller policy predicts a vector of length $Q$. At the stage $n$ of the lifelong process, the actual range of the skill index spans from 0 to $k_n$. \yifeng{Here, maybe we need an equation to represent casual masking.} To accommodate this, we apply a masking operation to the predicted vector, ensuring that, post-SoftMax application, the vector exclusively predicts skills within the actual range of this lifelong stage. 
Consistent with the training convention for skill policies, we utilize Experience Replay for the high-level meta-controller policy. Specifically, we leverage 5 demonstrations for previously learned tasks and 10 demonstrations for the newly introduced task to \cofinetune the meta-controller policy.

\todo{Explain why adding infinite values to softmax, instead of directly masking the output --- We need to make sure that the total probability sums up to 1, so adding infinite small value before softmax operation can meet this requirement while achieving masking, without the need to reweight the probability distributions by doing binary boolean masking on the output.}

==> tmp_ref.tex <==


@inproceedings{lan2015action,
  title={Action recognition by hierarchical mid-level action elements},
  author={Lan, Tian and Zhu, Yuke and Zamir, Amir Roshan and Savarese, Silvio},
  booktitle={ICCV},
  pages={4552--4560},
  year={2015}
}

@inproceedings{le2018hierarchical,
  title={Hierarchical imitation and reinforcement learning},
  author={Le, Hoang and Jiang, Nan and Agarwal, Alekh and Dud{\'\i}k, Miroslav and Yue, Yisong and Daum{\'e}, Hal},
  booktitle={ICML},
  pages={2917--2926},
  year={2018},
}

@article{yu2018one,
  title={One-shot hierarchical imitation learning of compound visuomotor tasks},
  author={Yu, Tianhe and Abbeel, Pieter and Levine, Sergey and Finn, Chelsea},
  journal={arXiv:1810.11043},
  year={2018}
}

@article{konidaris2009skill,
  title={Skill discovery in continuous reinforcement learning domains using skill chaining},
  author={Konidaris, George and Barto, Andrew},
  journal={NIPS},
  volume={22},
  pages={1015--1023},
  year={2009}
}

@inproceedings{konidaris2010constructing,
  title={Constructing Skill Trees for Reinforcement Learning Agents from Demonstration Trajectories.},
  author={Konidaris, George Dimitri and Kuindersma, Scott and Barto, Andrew G and Grupen, Roderic A},
  booktitle={NIPS},
  year={2010}
}

@inproceedings{niekum2012learning,
  title={Learning and generalization of complex tasks from unstructured demonstrations},
  author={Niekum, Scott and Osentoski, Sarah and Konidaris, George and Barto, Andrew G},
  booktitle={IROS},
  year={2012},
  organization={IEEE}
}

@inproceedings{mandlekar2020learning,
  title={Learning to generalize across long-horizon tasks from human demonstrations},
  author={Mandlekar, Ajay  and Xu, Danfei and Mart{\'\i}n-Mart{\'\i}n, Roberto and Savarese, Silvio and Fei-Fei, Li and Mandlekar, Ajay  and Xu, Danfei and Mart{\'\i}n-Mart{\'\i}n, Roberto and Savarese, Silvio and Fei-Fei, Li},
  booktitle={RSS},
  year={2020}
}

@inproceedings{mandlekar2020iris,
  title={Iris: Implicit reinforcement without interaction at scale for learning control from offline robot manipulation data},
  author={Mandlekar, Ajay and Ramos, Fabio and Boots, Byron and Savarese, Silvio and Fei-Fei, Li and Garg, Animesh and Fox, Dieter},
  booktitle={ICRA},
  year={2020},
  organization={IEEE}
}

@incollection{schaal2006dynamic,
  title={Dynamic movement primitives-a framework for motor control in humans and humanoid robotics},
  author={Schaal, Stefan},
  booktitle={Adaptive motion of animals and machines},
  pages={261--280},
  year={2006},
  publisher={Springer}
}


@inproceedings{shiarlis2018taco,
  title={Taco: Learning task decomposition via temporal alignment for control},
  author={Shiarlis, Kyriacos and Wulfmeier, Markus and Salter, Sasha and Whiteson, Shimon and Posner, Ingmar},
  booktitle={ICML},
  pages={4654--4663},
  year={2018},
}

@inproceedings{gupta2020relay,
  title={Relay Policy Learning: Solving Long-Horizon Tasks via Imitation and Reinforcement Learning},
  author={Gupta, Abhishek and Kumar, Vikash and Lynch, Corey and Levine, Sergey and Hausman, Karol},
  booktitle={CoRL},
  pages={1025--1037},
  year={2020},
}

@inproceedings{shankar2020learning,
  title={Learning robot skills with temporal variational inference},
  author={Shankar, Tanmay and Gupta, Abhinav},
  booktitle={ICML},
  pages={8624--8633},
  year={2020},
}

@article{zhu2020robosuite,
  title={robosuite: A modular simulation framework and benchmark for robot learning},
  author={Zhu, Yuke and Wong, Josiah and Mandlekar, Ajay and Mart{\'\i}n-Mart{\'\i}n, Roberto},
  journal={arXiv:2009.12293},
  year={2020}
}


@inproceedings{murali2016tsc,
  title={Tsc-dl: Unsupervised trajectory segmentation of multi-modal surgical demonstrations with deep learning},
  author={Murali, Adithyavairavan and Garg, Animesh and Krishnan, Sanjay and Pokorny, Florian T and Abbeel, Pieter and Darrell, Trevor and Goldberg, Ken},
  booktitle={ICRA},
  pages={4150--4157},
  year={2016},
  organization={IEEE}
}

@article{krishnan2017transition,
  title={Transition state clustering: Unsupervised surgical trajectory segmentation for robot learning},
  author={Krishnan, Sanjay and Garg, Animesh and Patil, Sachin and Lea, Colin and Hager, Gregory and Abbeel, Pieter and Goldberg, Ken},
  journal={IJRR},
  year={2017},
}

@inproceedings{lynch2020learning,
  title={Learning latent plans from play},
  author={Lynch, Corey and Khansari, Mohi and Xiao, Ted and Kumar, Vikash and Tompson, Jonathan and Levine, Sergey and Sermanet, Pierre},
  booktitle={CoRL},
  year={2020},
}

@inproceedings{tung2020learning,
  title={Learning Multi-Arm Manipulation Through Collaborative Teleoperation},
  author={Tung, Albert and Wong, Josiah and Mandlekar, Ajay and Mart{\'i}n-Mart{\'i}n, Roberto and Zhu, Yuke and Fei-Fei, Li and Savarese, Silvio},
  booktitle={ICRA},
  year={2021}
}

@article{tanneberg2021skid,
  title={SKID RAW: Skill Discovery from Raw Trajectories},
  author={Tanneberg, Daniel and Ploeger, Kai and Rueckert, Elmar and Peters, Jan},
  journal={RA-L},
  volume={6},
  number={3},
  pages={4696--4703},
  year={2021},
  publisher={IEEE}
}

@article{thrun1995lifelong,
  title={Lifelong robot learning},
  author={Thrun, Sebastian and Mitchell, Tom M},
  journal={Robotics and autonomous systems},
  volume={15},
  number={1-2},
  pages={25--46},
  year={1995},
  publisher={Elsevier}
}

@inproceedings{fei2016learning,
  title={Learning cumulatively to become more knowledgeable},
  author={Fei, Geli and Wang, Shuai and Liu, Bing},
  booktitle={Proceedings of the 22nd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
  pages={1565--1574},
  year={2016}
}

@article{Xie2021LifelongRR,
  title={Lifelong Robotic Reinforcement Learning by Retaining Experiences},
  author={Annie Xie and Chelsea Finn},
  journal={ArXiv},
  year={2021},
  volume={abs/2109.09180},
  url={https://api.semanticscholar.org/CorpusID:237572070}
}

@inproceedings{isele2018selective,
  title={Selective experience replay for lifelong learning},
  author={Isele, David and Cosgun, Akansel},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={32},
  number={1},
  year={2018}
}

@inproceedings{zhou2022forgetting,
  title={Forgetting and Imbalance in Robot Lifelong Learning with Off-policy Data},
  author={Zhou, Wenxuan and Bohez, Steven and Humplik, Jan and Heess, Nicolas and Abdolmaleki, Abbas and Rao, Dushyant and Wulfmeier, Markus and Haarnoja, Tuomas},
  booktitle={Conference on Lifelong Learning Agents},
  pages={294--309},
  year={2022},
  organization={PMLR}
}


@article{murtagh2012algorithms,
  title={Algorithms for hierarchical clustering: an overview},
  author={Murtagh, Fionn and Contreras, Pedro},
  journal={Wiley Interdisciplinary Reviews: Data Mining and Knowledge Discovery},
  volume={2},
  number={1},
  pages={86--97},
  year={2012},
  publisher={Wiley Online Library}
}

@article{rusu2016progressive,
  title={Progressive neural networks},
  author={Rusu, Andrei A and Rabinowitz, Neil C and Desjardins, Guillaume and Soyer, Hubert and Kirkpatrick, James and Kavukcuoglu, Koray and Pascanu, Razvan and Hadsell, Raia},
  journal={arXiv preprint arXiv:1606.04671},
  year={2016}
}

@inproceedings{gao2021cril,
  title={CRIL: Continual robot imitation learning via generative and prediction model},
  author={Gao, Chongkai and Gao, Haichuan and Guo, Shangqi and Zhang, Tianren and Chen, Feng},
  booktitle={2021 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={6747--5754},
  year={2021},
  organization={IEEE}
}

@article{kirkpatrick2017overcoming,
  title={Overcoming catastrophic forgetting in neural networks},
  author={Kirkpatrick, James and Pascanu, Razvan and Rabinowitz, Neil and Veness, Joel and Desjardins, Guillaume and Rusu, Andrei A and Milan, Kieran and Quan, John and Ramalho, Tiago and Grabska-Barwinska, Agnieszka and others},
  journal={Proceedings of the national academy of sciences},
  volume={114},
  number={13},
  pages={3521--3526},
  year={2017},
  publisher={National Acad Sciences}
}



@article{nair2019hierarchical,
  title={Hierarchical foresight: Self-supervised learning of long-horizon tasks via visual subgoal generation},
  author={Nair, Suraj and Finn, Chelsea},
  journal={arXiv:1909.05829},
  year={2019}
}

@inproceedings{andrychowicz2017hindsight,
  title={Hindsight experience replay},
  author={Andrychowicz, Marcin and Wolski, Filip and Ray, Alex and Schneider, Jonas and Fong, Rachel and Welinder, Peter and McGrew, Bob and Tobin, Josh and Abbeel, Pieter and Zaremba, Wojciech},
  booktitle={NIPS},
  year={2017}
}

@article{sutton1999between,
  title={Between MDPs and semi-MDPs: A framework for temporal abstraction in reinforcement learning},
  author={Sutton, Richard S and Precup, Doina and Singh, Satinder},
  journal={Artificial intelligence},
  volume={112},
  number={1-2},
  pages={181--211},
  year={1999},
  publisher={Elsevier}
}

@inproceedings{su2018learning,
  title={Learning manipulation graphs from demonstrations using multimodal sensory signals},
  author={Su, Zhe and Kroemer, Oliver and Loeb, Gerald E and Sukhatme, Gaurav S and Schaal, Stefan},
  booktitle={ICRA},
  year={2018},
  organization={IEEE}
}

@article{lee2020making,
  title={Making sense of vision and touch: Learning multimodal representations for contact-rich tasks},
  author={Lee, Michelle A and Zhu, Yuke and Zachares, Peter and Tan, Matthew and Srinivasan, Krishnan and Savarese, Silvio and Fei-Fei, Li and Garg, Animesh and Bohg, Jeannette},
  journal={IEEE Transactions on Robotics},
  year={2020},
}

@inproceedings{chu2019real,
  title={Real-time Multisensory Affordance-based Control for Adaptive Object Manipulation},
  author={Chu, Vivian and Gutierrez, Reymundo A and Chernova, Sonia and Thomaz, Andrea L and Chu, Vivian and Gutierrez, Reymundo A and Chernova, Sonia and Thomaz, Andrea L},
  booktitle={ICRA},
  year={2019},
  organization={IEEE}
}

@article{konidaris2019necessity,
  title={On the necessity of abstraction},
  author={Konidaris, George},
  journal={Current opinion in behavioral sciences},
  volume={29},
  pages={1--7},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{niekum2015online,
  title={Online bayesian changepoint detection for articulated motion models},
  author={Niekum, Scott and Osentoski, Sarah and Atkeson, Christopher G and Barto, Andrew G},
  booktitle={ICRA},
  year={2015},
  organization={IEEE}
}

@article{hinton2002training,
  title={Training products of experts by minimizing contrastive divergence},
  author={Hinton, Geoffrey E},
  journal={Neural computation},
  volume={14},
  number={8},
  pages={1771--1800},
  year={2002},
  publisher={MIT Press}
}



@article{fox2017multi,
  title={Multi-level discovery of deep options},
  author={Fox, Roy and Krishnan, Sanjay and Stoica, Ion and Goldberg, Ken},
  journal={arXiv:1703.08294},
  year={2017}
}

@inproceedings{xu2018neural,
  title={Neural task programming: Learning to generalize across hierarchical tasks},
  author={Xu, Danfei and Nair, Suraj and Zhu, Yuke and Gao, Julian and Garg, Animesh and Fei-Fei, Li and Savarese, Silvio},
  booktitle={ICRA},
  year={2018},
  organization={IEEE}
}

@inproceedings{huang2019neural,
  title={Neural task graphs: Generalizing to unseen tasks from a single video demonstration},
  author={Huang, De-An and Nair, Suraj and Xu, Danfei and Zhu, Yuke and Garg, Animesh and Fei-Fei, Li and Savarese, Silvio and Niebles, Juan Carlos},
  booktitle={CVPR},
  pages={8565--8574},
  year={2019}
}


@inproceedings{kaelbling2011hierarchical,
  title={Hierarchical task and motion planning in the now},
  author={Kaelbling, Leslie Pack and Lozano-P{\'e}rez, Tom{\'a}s},
  booktitle={ICRA},
  year={2011},
  organization={IEEE}
}

@article{garrett2021integrated,
  title={Integrated task and motion planning},
  author={Garrett, Caelan Reed and Chitnis, Rohan and Holladay, Rachel and Kim, Beomjoon and Silver, Tom and Kaelbling, Leslie Pack and Lozano-P{\'e}rez, Tom{\'a}s},
  journal={Annual review of control, robotics, and autonomous systems},
  volume={4},
  pages={265--293},
  year={2021},
  publisher={Annual Reviews}
}

@article{kaelbling2013integrated,
  title={Integrated task and motion planning in belief space},
  author={Kaelbling, Leslie Pack and Lozano-P{\'e}rez, Tom{\'a}s},
  journal={IJRR},
  volume={32},
  number={9-10},
  pages={1194--1227},
  year={2013},
  publisher={Sage Publications Sage UK: London, England}
}

@incollection{reddy2018survey,
  title={A survey of partitional and hierarchical clustering algorithms},
  author={Reddy, Chandan K and Vinzamuri, Bhanukiran},
  booktitle={Data clustering},
  pages={87--110},
  year={2018},
  publisher={Chapman and Hall/CRC}
}


@article{sarfraz2021temporally,
  title={Temporally-Weighted Hierarchical Clustering for Unsupervised Action Segmentation},
  author={Sarfraz, M Saquib and Murray, Naila and Sharma, Vivek and Diba, Ali and Van Gool, Luc and Stiefelhagen, Rainer},
  journal={arXiv:2103.11264},
  year={2021}
}


@inproceedings{sarfraz2019efficient,
  title={Efficient parameter-free clustering using first neighbor relations},
  author={Sarfraz, Saquib and Sharma, Vivek and Stiefelhagen, Rainer},
  booktitle={CVPR},
  year={2019}
}
@article{kingma2013auto,
  title={Auto-encoding variational bayes},
  author={Kingma, Diederik P and Welling, Max},
  journal={arXiv:1312.6114},
  year={2013}
}

@article{zacks2001event,
  title={Event structure in perception and conception},
  author={Zacks, Jeffrey M and Tversky, Barbara},
  journal={Psychological bulletin},
  volume={127},
  number={1},
  pages={3},
  year={2001},
  publisher={American Psychological Association}
}



@inproceedings{zhang2018deep,
  title={Deep imitation learning for complex manipulation tasks from virtual reality teleoperation},
  author={Zhang, Tianhao and McCarthy, Zoe and Jow, Owen and Lee, Dennis and Chen, Xi and Goldberg, Ken and Abbeel, Pieter},
  booktitle={ICRA},
  year={2018},
}


@article{khatib1987unified,
  title={A unified approach for motion and force control of robot manipulators: The operational space formulation},
  author={Khatib, Oussama},
  journal={IEEE Journal on Robotics and Automation},
  volume={3},
  number={1},
  pages={43--53},
  year={1987},
  publisher={IEEE}
}


@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={CVPR},
  year={2016}
}

@inproceedings{finn2016deep,
  title={Deep spatial autoencoders for visuomotor learning},
  author={Finn, Chelsea and Tan, Xin Yu and Duan, Yan and Darrell, Trevor and Levine, Sergey and Abbeel, Pieter},
  booktitle={ICRA},
  year={2016},
  organization={IEEE}
}


@article{kostrikov2020image,
  title={Image augmentation is all you need: Regularizing deep reinforcement learning from pixels},
  author={Kostrikov, Ilya and Yarats, Denis and Fergus, Rob},
  journal={arXiv:2004.13649},
  year={2020}
}

@inproceedings{bagaria2019option,
  title={Option discovery using deep skill chaining},
  author={Bagaria, Akhil and Konidaris, George},
  booktitle={ICLR},
  year={2019}
}



@inproceedings{dietterich1998maxq,
  title={The {MAXQ} Method for Hierarchical Reinforcement Learning.},
  author={Dietterich, Thomas G},
  booktitle={ICML},
  volume={98},
  year={1998},
}



@inproceedings{vezhnevets2017feudal,
  title={Feudal networks for hierarchical reinforcement learning},
  author={Vezhnevets, Alexander Sasha and Osindero, Simon and Schaul, Tom and Heess, Nicolas and Jaderberg, Max and Silver, David and Kavukcuoglu, Koray},
  booktitle={ICML},
  year={2017},
}


@inproceedings{kumar2018expanding,
  title={Expanding motor skills using relay networks},
  author={Kumar, Visak CV and Ha, Sehoon and Liu, C Karen},
  booktitle={CoRL},
  year={2018},
}

@inproceedings{henderson2018optiongan,
  title={Optiongan: Learning joint reward-policy options using generative adversarial inverse reinforcement learning},
  author={Henderson, Peter and Chang, Wei-Di and Bacon, Pierre-Luc and Meger, David and Pineau, Joelle and Precup, Doina},
  booktitle={AAAI},
  volume={32},
  number={1},
  year={2018}
}


@article{stulp2012reinforcement,
  title={Reinforcement learning with sequences of motion primitives for robust manipulation},
  author={Stulp, Freek and Theodorou, Evangelos A and Schaal, Stefan},
  journal={IEEE Transactions on robotics},
  volume={28},
  number={6},
  pages={1360--1370},
  year={2012},
  publisher={IEEE}
}


@article{gregor2016variational,
  title={Variational intrinsic control},
  author={Gregor, Karol and Rezende, Danilo Jimenez and Wierstra, Daan},
  journal={arXiv:1611.07507},
  year={2016}
}

@inproceedings{sharma2019dynamics,
  title={Dynamics-Aware Unsupervised Discovery of Skills},
  author={Sharma, Archit and Gu, Shixiang and Levine, Sergey and Kumar, Vikash and Hausman, Karol},
  booktitle={ICLR},
  year={2019}
}

@article{jiang2022vima,
  title={Vima: General robot manipulation with multimodal prompts},
  author={Jiang, Yunfan and Gupta, Agrim and Zhang, Zichen and Wang, Guanzhi and Dou, Yongqiang and Chen, Yanjun and Fei-Fei, Li and Anandkumar, Anima and Zhu, Yuke and Fan, Linxi},
  journal={arXiv preprint arXiv:2210.03094},
  year={2022}
}

@inproceedings{daniel2012hierarchical,
  title={Hierarchical relative entropy policy search},
  author={Daniel, Christian and Neumann, Gerhard and Peters, Jan},
  booktitle={Artificial Intelligence and Statistics},
  pages={273--281},
  year={2012},
}

@article{eysenbach2018diversity,
  title={Diversity is all you need: Learning skills without a reward function},
  author={Eysenbach, Benjamin and Gupta, Abhishek and Ibarz, Julian and Levine, Sergey},
  journal={arXiv:1802.06070 },
  year={2018}
}


@inproceedings{hausman2018learning,
  title={Learning an embedding space for transferable robot skills},
  author={Hausman, Karol and Springenberg, Jost Tobias and Wang, Ziyu and Heess, Nicolas and Riedmiller, Martin},
  booktitle={ICLR},
  year={2018}
}

@book{gibson1966senses,
  title={The senses considered as perceptual systems},
  author={Gibson, James Jerome and Carmichael, Leonard},
  volume={2},
  number={1},
  year={1966},
  publisher={Houghton Mifflin Boston}
}

@inproceedings{zhou2019bottom,
  title={Bottom-up object detection by grouping extreme and center points},
  author={Zhou, Xingyi and Zhuo, Jiacheng and Krahenbuhl, Philipp},
  booktitle={CVPR},
  pages={850--859},
  year={2019}
}

@inproceedings{law2018cornernet,
  title={Cornernet: Detecting objects as paired keypoints},
  author={Law, Hei and Deng, Jia},
  booktitle={ECCV},
  year={2018}
}

@inproceedings{newell2016stacked,
  title={Stacked hourglass networks for human pose estimation},
  author={Newell, Alejandro and Yang, Kaiyu and Deng, Jia},
  booktitle={ECCV},
  year={2016},
}


@article{brooks1991intelligence,
  title={Intelligence without representation},
  author={Brooks, Rodney A},
  journal={Artificial Intelligence},
  volume={47},
  number={1-3},
  pages={139--159},
  year={1991},
}


@article{brooks1986robust,
  title={A robust layered control system for a mobile robot},
  author={Brooks, Rodney},
  journal={IEEE Journal on Robotics and Automation},
  volume={2},
  number={1},
  pages={14--23},
  year={1986},
}

@inproceedings{nicolescu2002hierarchical,
  title={A hierarchical architecture for behavior-based robots},
  author={Nicolescu, Monica N and Matari{\'c}, Maja J},
  booktitle={AAMAS},
  year={2002}
}


@article{pirk2020modeling,
  title={Modeling Long-horizon Tasks as Sequential Interaction Landscapes},
  author={Pirk, S{\"o}ren and Hausman, Karol and Toshev, Alexander and Khansari, Mohi},
  journal={arXiv:2006.04843},
  year={2020}
}

@article{duan2017one,
  title={One-shot imitation learning},
  author={Duan, Yan and Andrychowicz, Marcin and Stadie, Bradly C and Ho, Jonathan and Schneider, Jonas and Sutskever, Ilya and Abbeel, Pieter and Zaremba, Wojciech},
  journal={arXiv:1703.07326},
  year={2017}
}

@article{smith2019avid,
  title={Avid: Learning multi-stage tasks via pixel-level translation of human videos},
  author={Smith, Laura and Dhawan, Nikita and Zhang, Marvin and Abbeel, Pieter and Levine, Sergey},
  journal={arXiv:1912.04443},
  year={2019}
}

@article{farag2016bottom,
  title={A bottom-up approach for pancreas segmentation using cascaded superpixels and (deep) image patch labeling},
  author={Farag, Amal and Lu, Le and Roth, Holger R and Liu, Jiamin and Turkbey, Evrim and Summers, Ronald M},
  journal={IEEE Transactions on Image Processing},
  volume={26},
  number={1},
  pages={386--399},
  year={2016},
  publisher={IEEE}
}

@article{kipf2018compositional,
  title={Compositional imitation learning: Explaining and executing one task at a time},
  author={Kipf, Thomas and Li, Yujia and Dai, Hanjun and Zambaldi, Vinicius and Grefenstette, Edward and Kohli, Pushmeet and Battaglia, Peter},
  journal={arXiv:1812.01483},
  year={2018}
}

@article{von2007tutorial,
  title={A tutorial on spectral clustering},
  author={Von Luxburg, Ulrike},
  journal={Statistics and computing},
  volume={17},
  number={4},
  pages={395--416},
  year={2007},
  publisher={Springer}
}

@inproceedings{schaul2015universal,
  title={Universal value function approximators},
  author={Schaul, Tom and Horgan, Daniel and Gregor, Karol and Silver, David},
  booktitle={ICML},
  year={2015},
}

@article{konidaris2018skills,
  title={From skills to symbols: Learning symbolic representations for abstract high-level planning},
  author={Konidaris, George and Kaelbling, Leslie Pack and Lozano-Perez, Tomas},
  journal={Journal of Artificial Intelligence Research},
  volume={61},
  pages={215--289},
  year={2018}
}

@article{van2008visualizing,
  title={Visualizing data using t-SNE.},
  author={Van der Maaten, Laurens and Hinton, Geoffrey},
  journal={Journal of machine learning research},
  volume={9},
  number={11},
  year={2008}
}

@MISC{Precup00temporalabstraction,
    author = {Doina Precup},
    title = {Temporal Abstraction in Reinforcement Learning},
    year = {2000}
}

@inproceedings{hovland1996skill,
  title={Skill acquisition from human demonstration using a hidden markov model},
  author={Hovland, Geir E and Sikka, Pavan and McCarragher, Brenan J},
  booktitle={ICRA},
  volume={3},
  year={1996},
}


@article{liu2023libero,
  title={LIBERO: Benchmarking Knowledge Transfer for Lifelong Robot Learning},
  author={Liu, Bo and Zhu, Yifeng and Gao, Chongkai and Feng, Yihao and Liu, Qiang and Zhu, Yuke and Stone, Peter},
  journal={arXiv preprint arXiv:2306.03310},
  year={2023}
}


@article{zhu2022bottom,
  title={Bottom-up skill discovery from unsegmented demonstrations for long-horizon robot manipulation},
  author={Zhu, Yifeng and Stone, Peter and Zhu, Yuke},
  journal={IEEE Robotics and Automation Letters},
  volume={7},
  number={2},
  pages={4126--4133},
  year={2022},
  publisher={IEEE}
}


@article{zhu2022viola,
  title={VIOLA: Imitation Learning for Vision-Based Manipulation with Object Proposal Priors},
  author={Zhu, Yifeng and Joshi, Abhishek and Stone, Peter and Zhu, Yuke},
  journal={arXiv preprint arXiv:2210.11339},
  year={2022}
}

@article{devlin2018bert,
  title={Bert: Pre-training of deep bidirectional transformers for language understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  journal={arXiv preprint arXiv:1810.04805},
  year={2018}
}

@inproceedings{perez2018film,
  title={Film: Visual reasoning with a general conditioning layer},
  author={Perez, Ethan and Strub, Florian and De Vries, Harm and Dumoulin, Vincent and Courville, Aaron},
  booktitle={Proceedings of the AAAI conference on artificial intelligence},
  volume={32},
  number={1},
  year={2018}
}

@article{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@article{bishop1994mixture,
  title={Mixture density networks},
  author={Bishop, Christopher M},
  year={1994},
  publisher={Aston University}
}

@article{mandlekar2021matters,
  title={What matters in learning from offline human demonstrations for robot manipulation},
  author={Mandlekar, Ajay and Xu, Danfei and Wong, Josiah and Nasiriany, Soroush and Wang, Chen and Kulkarni, Rohun and Fei-Fei, Li and Savarese, Silvio and Zhu, Yuke and Mart{\'\i}n-Mart{\'\i}n, Roberto},
  journal={arXiv preprint arXiv:2108.03298},
  year={2021}
}

@inproceedings{grauman2022ego4d,
  title={Ego4d: Around the world in 3,000 hours of egocentric video},
  author={Grauman, Kristen and Westbury, Andrew and Byrne, Eugene and Chavis, Zachary and Furnari, Antonino and Girdhar, Rohit and Hamburger, Jackson and Jiang, Hao and Liu, Miao and Liu, Xingyu and others},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={18995--19012},
  year={2022}
}

@article{nasiriany2022learning,
  title={Learning and retrieval from prior data for skill-based imitation learning},
  author={Nasiriany, Soroush and Gao, Tian and Mandlekar, Ajay and Zhu, Yuke},
  journal={arXiv preprint arXiv:2210.11435},
  year={2022}
}

@inproceedings{pertsch2021accelerating,
  title={Accelerating reinforcement learning with learned skill priors},
  author={Pertsch, Karl and Lee, Youngwoon and Lim, Joseph},
  booktitle={Conference on robot learning},
  pages={188--204},
  year={2021},
  organization={PMLR}
}

@article{oquab2023dinov2,
  title={Dinov2: Learning robust visual features without supervision},
  author={Oquab, Maxime and Darcet, Timoth{\'e}e and Moutakanni, Th{\'e}o and Vo, Huy and Szafraniec, Marc and Khalidov, Vasil and Fernandez, Pierre and Haziza, Daniel and Massa, Francisco and El-Nouby, Alaaeldin and others},
  journal={arXiv preprint arXiv:2304.07193},
  year={2023}
}

@inproceedings{radford2021learning,
  title={Learning transferable visual models from natural language supervision},
  author={Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and others},
  booktitle={International conference on machine learning},
  pages={8748--8763},
  year={2021},
  organization={PMLR}
}

@article{minderer2022simple,
  title={Simple Open-Vocabulary Object Detection with Vision Transformers},
  author={Matthias, Minderer and Alexey, Gritsenko and Austin, Stone and Maxim, Neumann and Dirk, Weissenborn and Alexey, Dosovitskiy and Aravindh, Mahendran and Anurag, Arnab and Mostafa, Dehghani and Zhuoran, Shen and Xiao, Wang and Xiaohua, Zhai and Thomas, Kipf and Neil Houlsby},
  journal={ECCV},
  year={2022},
}

@article{rousseeuw1987silhouettes,
  title={Silhouettes: a graphical aid to the interpretation and validation of cluster analysis},
  author={Rousseeuw, Peter J},
  journal={Journal of computational and applied mathematics},
  volume={20},
  pages={53--65},
  year={1987},
  publisher={Elsevier}
}

@article{chaudhry2019tiny,
  title={On tiny episodic memories in continual learning},
  author={Chaudhry, Arslan and Rohrbach, Marcus and Elhoseiny, Mohamed and Ajanthan, Thalaiyasingam and Dokania, Puneet K and Torr, Philip HS and Ranzato, Marc'Aurelio},
  journal={arXiv preprint arXiv:1902.10486},
  year={2019}
}

@article{diaz2018don,
  title={Don't forget, there is more than forgetting: new metrics for Continual Learning},
  author={D{\'\i}az-Rodr{\'\i}guez, Natalia and Lomonaco, Vincenzo and Filliat, David and Maltoni, Davide},
  journal={arXiv preprint arXiv:1810.13166},
  year={2018}
}

@inproceedings{bain1995framework,
  title={A Framework for Behavioural Cloning.},
  author={Bain, Michael and Sammut, Claude},
  booktitle={Machine Intelligence 15},
  pages={103--129},
  year={1995}
}

@article{nair2022r3m,
  title={R3m: A universal visual representation for robot manipulation},
  author={Nair, Suraj and Rajeswaran, Aravind and Kumar, Vikash and Finn, Chelsea and Gupta, Abhinav},
  journal={arXiv preprint arXiv:2203.12601},
  year={2022}
}

@article{duan2017one,
  title={One-shot imitation learning},
  author={Duan, Yan and Andrychowicz, Marcin and Stadie, Bradly and Jonathan Ho, OpenAI and Schneider, Jonas and Sutskever, Ilya and Abbeel, Pieter and Zaremba, Wojciech},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@inproceedings{finn2017one,
  title={One-shot visual imitation learning via meta-learning},
  author={Finn, Chelsea and Yu, Tianhe and Zhang, Tianhao and Abbeel, Pieter and Levine, Sergey},
  booktitle={Conference on robot learning},
  pages={357--368},
  year={2017},
  organization={PMLR}
}

@inproceedings{mandi2022towards,
  title={Towards more generalizable one-shot visual imitation learning},
  author={Mandi, Zhao and Liu, Fangchen and Lee, Kimin and Abbeel, Pieter},
  booktitle={2022 International Conference on Robotics and Automation (ICRA)},
  pages={2434--2444},
  year={2022},
  organization={IEEE}
}

@inproceedings{lynch2020learning,
  title={Learning latent plans from play},
  author={Lynch, Corey and Khansari, Mohi and Xiao, Ted and Kumar, Vikash and Tompson, Jonathan and Levine, Sergey and Sermanet, Pierre},
  booktitle={Conference on robot learning},
  pages={1113--1132},
  year={2020},
  organization={PMLR}
}

@inproceedings{shiarlis2018taco,
  title={Taco: Learning task decomposition via temporal alignment for control},
  author={Shiarlis, Kyriacos and Wulfmeier, Markus and Salter, Sasha and Whiteson, Shimon and Posner, Ingmar},
  booktitle={International Conference on Machine Learning},
  pages={4654--4663},
  year={2018},
  organization={PMLR}
}

@article{wang2023voyager,
  title={Voyager: An open-ended embodied agent with large language models},
  author={Wang, Guanzhi and Xie, Yuqi and Jiang, Yunfan and Mandlekar, Ajay and Xiao, Chaowei and Zhu, Yuke and Fan, Linxi and Anandkumar, Anima},
  journal={arXiv preprint arXiv:2305.16291},
  year={2023}
}

@article{mendez2023embodied,
  title={Embodied Lifelong Learning for Task and Motion Planning},
  author={Mendez, Jorge A and Kaelbling, Leslie Pack and Lozano-P{\'e}rez, Tom{\'a}s},
  journal={arXiv preprint arXiv:2307.06870},
  year={2023}
}

@article{kirkpatrick2017overcoming,
  title={Overcoming catastrophic forgetting in neural networks},
  author={Kirkpatrick, James and Pascanu, Razvan and Rabinowitz, Neil and Veness, Joel and Desjardins, Guillaume and Rusu, Andrei A and Milan, Kieran and Quan, John and Ramalho, Tiago and Grabska-Barwinska, Agnieszka and others},
  journal={Proceedings of the national academy of sciences},
  volume={114},
  number={13},
  pages={3521--3526},
  year={2017},
  publisher={National Acad Sciences}
}

@inproceedings{zenke2017continual,
  title={Continual learning through synaptic intelligence},
  author={Zenke, Friedemann and Poole, Ben and Ganguli, Surya},
  booktitle={International conference on machine learning},
  pages={3987--3995},
  year={2017},
  organization={PMLR}
}

@article{li2017learning,
  title={Learning without forgetting},
  author={Li, Zhizhong and Hoiem, Derek},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={40},
  number={12},
  pages={2935--2947},
  year={2017},
  publisher={IEEE}
}

@article{nguyen2017variational,
  title={Variational continual learning},
  author={Nguyen, Cuong V and Li, Yingzhen and Bui, Thang D and Turner, Richard E},
  journal={arXiv preprint arXiv:1710.10628},
  year={2017}
}

@article{powers2023evaluating,
  title={Evaluating Continual Learning on a Home Robot},
  author={Powers, Sam and Gupta, Abhinav and Paxton, Chris},
  journal={arXiv preprint arXiv:2306.02413},
  year={2023}
}

@article{lopez2017gradient,
  title={Gradient episodic memory for continual learning},
  author={Lopez-Paz, David and Ranzato, Marc'Aurelio},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@article{mendez2022modular,
  title={Modular lifelong reinforcement learning via neural composition},
  author={Mendez, Jorge A and van Seijen, Harm and Eaton, Eric},
  journal={arXiv preprint arXiv:2207.00429},
  year={2022}
}

@article{ben2022lifelong,
  title={Lifelong reinforcement learning with modulating masks},
  author={Ben-Iwhiwhu, Eseoghene and Nath, Saptarshi and Pilly, Praveen K and Kolouri, Soheil and Soltoggio, Andrea},
  journal={arXiv preprint arXiv:2212.11110},
  year={2022}
}

@inproceedings{xie2022lifelong,
  title={Lifelong robotic reinforcement learning by retaining experiences},
  author={Xie, Annie and Finn, Chelsea},
  booktitle={Conference on Lifelong Learning Agents},
  pages={838--855},
  year={2022},
  organization={PMLR}
}

@article{xie2020deep,
  title={Deep reinforcement learning amidst lifelong non-stationarity},
  author={Xie, Annie and Harrison, James and Finn, Chelsea},
  journal={arXiv preprint arXiv:2006.10701},
  year={2020}
}

@article{xie2020deep2,
  title={Deep imitation learning for bimanual robotic manipulation},
  author={Xie, Fan and Chowdhury, Alexander and De Paolis Kaluza, M and Zhao, Linfeng and Wong, Lawson and Yu, Rose},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={2327--2337},
  year={2020}
}

@article{raghavan2020lifelong,
  title={Lifelong learning using eigentasks: Task separation, skill acquisition, and selective transfer},
  author={Raghavan, Aswin and Hostetler, Jesse and Sur, Indranil and Rahman, Abrar and Divakaran, Ajay},
  journal={arXiv preprint arXiv:2007.06918},
  year={2020}
}


@article{wu2020model,
  title={Model primitives for hierarchical lifelong reinforcement learning},
  author={Wu, Bohan and Gupta, Jayesh K and Kochenderfer, Mykel},
  journal={Autonomous Agents and Multi-Agent Systems},
  volume={34},
  pages={1--38},
  year={2020},
  publisher={Springer}
}

@article{shafiullah2022one,
  title={One after another: Learning incremental skills for a changing world},
  author={Shafiullah, Nur Muhammad and Pinto, Lerrel},
  journal={arXiv preprint arXiv:2203.11176},
  year={2022}
}

@inproceedings{tessler2017deep,
  title={A deep hierarchical approach to lifelong learning in minecraft},
  author={Tessler, Chen and Givony, Shahar and Zahavy, Tom and Mankowitz, Daniel and Mannor, Shie},
  booktitle={Proceedings of the AAAI conference on artificial intelligence},
  volume={31},
  number={1},
  year={2017}
}

@article{wang2023comprehensive,
  title={A comprehensive survey of continual learning: Theory, method and application},
  author={Wang, Liyuan and Zhang, Xingxing and Su, Hang and Zhu, Jun},
  journal={arXiv preprint arXiv:2302.00487},
  year={2023}
}

@inproceedings{shah2023mutex,
    title={{MUTEX}: Learning Unified Policies from Multimodal Task Specifications},
    author={Rutav Shah and Roberto Mart{\'\i}n-Mart{\'\i}n and Yuke Zhu},
    booktitle={7th Annual Conference on Robot Learning},
    year={2023}
}

@inproceedings{zhu2023learning,
  title={Learning Generalizable Manipulation Policies with Object-Centric 3D Representations},
  author={Zhu, Yifeng and Jiang, Zhenyu and Stone, Peter and Zhu, Yuke},
  booktitle={7th Annual Conference on Robot Learning},
  year={2023},
}
@inproceedings{mallya2018packnet,
  title={Packnet: Adding multiple tasks to a single network by iterative pruning},
  author={Mallya, Arun and Lazebnik, Svetlana},
  booktitle={Proceedings of the IEEE conference on Computer Vision and Pattern Recognition},
  pages={7765--7773},
  year={2018}
}

@article{fu2022meta,
  title={Meta-Learning Transferable Parameterized Skills},
  author={Fu, Haotian and Yu, Shangqun and Tiwari, Saket and Konidaris, George and Littman, Michael},
  journal={arXiv preprint arXiv:2206.03597},
  year={2022}
}

@article{wang2023mimicplay,
  title={Mimicplay: Long-horizon imitation learning by watching human play},
  author={Wang, Chen and Fan, Linxi and Sun, Jiankai and Zhang, Ruohan and Fei-Fei, Li and Xu, Danfei and Zhu, Yuke and Anandkumar, Anima},
  journal={arXiv preprint arXiv:2302.12422},
  year={2023}
}

@misc{vonluxburg2007tutorial,
      title={A Tutorial on Spectral Clustering}, 
      author={Ulrike von Luxburg},
      year={2007},
      eprint={0711.0189},
      archivePrefix={arXiv},
      primaryClass={cs.DS}
}

@article{chi2023diffusion,
  title={Diffusion policy: Visuomotor policy learning via action diffusion},
  author={Chi, Cheng and Feng, Siyuan and Du, Yilun and Xu, Zhenjia and Cousineau, Eric and Burchfiel, Benjamin and Song, Shuran},
  journal={arXiv preprint arXiv:2303.04137},
  year={2023}
}

@article{luo2023multi,
  title={Multi-Stage Cable Routing through Hierarchical Imitation Learning},
  author={Luo, Jianlan and Xu, Charles and Geng, Xinyang and Feng, Gilbert and Fang, Kuan and Tan, Liam and Schaal, Stefan and Levine, Sergey},
  journal={arXiv preprint arXiv:2307.08927},
  year={2023}
}
